Distributed anonymous discrete function computation

We propose a model for deterministic distributed function computation by a network of identical and anonymous nodes. In this model, each node has bounded computation and storage capabilities that do not grow with the network size. Furthermore, each node only knows its neighbors, not the entire graph. Our goal is to characterize the class of functions that can be computed within this model. In our main result, we provide a necessary condition for computability which we show to be nearly sufficient, in the sense that every function that satisfies this condition can at least be approximated. The problem of computing suitably rounded averages in a distributed manner plays a central role in our development; we provide an algorithm that solves it in time that grows quadratically with the size of the network.

==> appen_formal_proof.tex <==
\newpage
\appendix
\section{\rt{More detailed proofs of some lemmas}}


\comjh{The present appendix contains more detailed proofs of some
lemmas of Section \ref{sec:comput_average}. It is not meant to be
included in the paper as such and would probably need some re-writing before (if?) publication. The options are\\
%
- to keep the proofs for ourself us and let the rest of the paper
in its
present form\\
- to add these proofs in an appendix of the paper or of an
extended version of it \\
- to add in the paper a reference to an url with the proofs\\
- to include the proofs in the paper. \\\\
Note: there might exist some simplifications }





\subsection{Lemma \ref{lem:descr_Gr}}



\begin{lemma}%\label{lem:descr_Gr}
The graph $G_r$(t) consists of a set of non intersecting directed
simple\footnote{By simple path we mean a path containing at most
once every node and edge}
paths. For each maximal path, the following hold:\\
\begin{itemize}
\item{The root node $r$ has $Rin_r(t) = r$ and has initiated a
request at a time $t'\leq t$ and received no answer yet.}%
\item{The end node $s$ has $Rout_s(t) \not = s$. There is either a
request transmission from $s$ to $Rout_s(t)$ or an answer to a
request from $Rout_s(t)$ to $s$.}
\end{itemize}
\end{lemma}
\begin{proof}


\emph{(a1) If $Rin_j(t) =i\neq j$, then there holds $Rout_i(t)
=Rout_i(t-1)= j$, and therefore $(i,j)\in G_r(t)$.}\\

Initially, every $j$ is in free mode and no $Rin_j$ is thus
defined. Suppose now that the results holds until $t-1$, and
consider a pair $i,j$ of vertices at time $t$, so that $Rin_j(t) =
i$.

If $Rin_j(t-1) =i$, then by induction hypothesis there holds
$Rout_i(t-1)=j$, and both $i$ and $j$ are blocked at time $t-1$.
Therefore, there was no "answer to a request" from $j$ to $i$ at
time $t-1$ for this would have required $j$ to execute "transmit
answer" or "answer request" at time $t-2$, letting it in a free
mode at time $t-1$. As a result, $i$ cannot execute any operation
at time $t-1$, so that $Rout_i(t) = Rout_i(t-1) = j$.

Suppose now that $Rin_j(t-1) \not = i$. The only operation
allowing to set $Rin_j(t)$ to some $i\not =j$ is "transmit
request", and can be executed at time $t-1$ only if $j$ reads a
request sent/transmitted by $i$ at time $t-2$. The two operations
during which $i$ could transmit/emit a request are "transmit
request" and "emit request". Both also set $Rout_i(t-1)=j$ and the
mode of $i$ to "blocked". There remains to prove that $i$ does not
change $Rout_i(t)$ at time $t-1$. Since $i$ is in a blocked mode
at time $t-1$, changing $Rout$ would require executing "transmit
answer" or "receive answer", which can only be done after reading
an answer message from $Rout_i(t-1) =j$. This message should have
been sent by $j$ at time $t-2$, and would have required either
$Rin_j(t-2) =i$ (operation "transmit answer"), or $j$ to have read
a request emitted/transmitted by $i$ at time $t-3$. In the first
case, the induction hypothesis implies that $Rout_i(t-2) =j$. This
also holds in the second case, as when $i$ emits a request to $j$
it sets $Rout_i(t-2) = j$. This implies that $i$ is in a blocked
mode at time $t-2$ because $Rout_i$ is not defined in free mode,
and therefore that it cannot emit/transmit a request to $i$ at
that time.

\bigskip

\emph{(a2) The graph is acyclic.}\\

If an edge $(i,j)$ appears at time $t$, since $Rin_j(t) =i$, we
must have $Rout_i(t) =Rout_i(t-1)= j$ by (a1), and therefore
$Rin_j(t-1) \not = i$ for otherwise the edge would already have
been present at time $t-1$. The only operation by which $j$ can
set $Rin_j(t)$ to another node is "transmit request", and it
requires $j$ to be in a free mode at time $t-1$, and thus to have
$Rout_j(t-1) = \emptyset$. We have seen (a1) that this implies
that no node $k$ can have $Rin_k(t) = j$, so that no edge can
leave $j$ at time $t$. So when an edge appears in $G_r$, its
endpoint has an out-degree 0, and no cycle can thus appear. This
proves the acyclicity of the graph since it is initially empty.

\bigskip

\emph{(a3) The graph $G_r$(t) consists of a set of non
intersecting directed simple paths.}\\

It follows directly from the definition of the graph that the out-
and in-degrees of the nodes are bounded by 1. Combined with (a2),
this implies (a3)

\bigskip

\emph{(a4) The root node $r$ (of a maximal path) has $Rin_r(t) =
r$ and has initiated a request at a time $t'\leq t$ and received
no answer yet.}\\

Since $r$ is in the graph it must have a nonempty $Rin_r(t)$, and
it follows from (a1) that $Rin_r(t)$ is not another node because
$r$ has no incoming edge, so there must hold $Rin_r(t)=r$. Observe
now that the only way for $r$ to set $Rin_r$ to itself is to
execute "emit request" at some time $t'<t$. Moreover, since the
last request emission, it has not executed "receive answer", for
this would have set $Rin_r$ to void.

\bigskip

\emph{(a5) The end node $s$ has $Rout_s(t) \not = s$. There is
either a request transmission from $s$ to $Rout_s(t)$ or an answer
to a request from $Rout_s(t)$ to $s$.}\\

Suppose that $s\not = r$. By hypothesis, $Rin_s(t) \not =s$. The
only way to set $Rin_s$ to another node is to execute "transmit
request", and it automatically sets $Rout_s$ to another node $k$
after sending it a request, and sets $s$ in blocked mode. Let $t'$
be the last time at which it has executed this operation. Since
$t'$, $s$ did not change $Rin_s$ and did thus not execute
"transmit answer" (nor "receive answer"). It is thus still in a
blocked mode, and has not changed $Rout_s=k$ either. On the other
hand, we know that $Rin_k(t)$ is not $s$, for otherwise there
would be an edge $(s,k)$ in $G_r(t)$.

If $t=t'+1$, the the result trivially because of the request that
$s$ has sent at time $t'$ (which is thus present at time $t'+1$).
Suppose now that $t>t'+1$, and that $k$ has denied the request at
time $t'+1$. In that case, there is a (negative) answer from $k$
to $s$ at time $t'+2$, leading $s$ to execute "transmit answer" at
time $t'+2$ so that it is again in a free mode with $Rin_s$
undefined at $t'+3$. So the only $t$ that does not contradict our
assumptions is $t'+2$, and the result holds in that case. Finally
$k$ could have transmitted the request to a further node. In that
case, it sets $Rin_k(t'+2)$ to $s$ and entered a blocked mode.
Since $Rin_k(t)$ is now different from $s$, and $s$ has not
changed $Rout_s(t)$, the only possibility is that at time $t-1$
node $k$ has executed "transmit answer", so that there is an
answer arriving at $s$ at time $t$. The results holds thus also in
that case, and a similar analysis is valid if $s=r$.

\end{proof}





\subsection{Lemma \ref{lem:request_terminate}}




\begin{lemma}
If a node is in blocked mode at time $t'$, then it belongs to a
maximal path $\mathcal{P}_r(t')$ in $G_r(t')$, for some starting
node $r$. Moreover, there exists $t_e<t_a<t_f$ with $t'\in
[t_e,t_f]$, and $t_f-t_a = t_a -t_e \leq n$ such that
\begin{itemize}
\item{Node $r$ executes "emit request" at time $t_e$, there is a
trivial path of length 0 staring from $r$ at time $t_e+1$, and the
request contains the value $\rt{u}_i(t_e)$.}
%
\item{For every $t\int [t_e+1,t_a-1]$, there is a request from the
last node of the path $s_r(t)$ to $Rout_{s_r(t)}(t)$ with the
value $\rt{u}_i(t_e)$, and there holds $\mathcal{P}_r(t+1) =
\mathcal{P}_r(t) \cup Rout_{s(t)}(t)$, i.e., the request will be
transmitted at the next time step, and $Rout_{s_r(t)}$ will join
the the request path}
%
\item{At time $t_a$, $Rout_{s_r(t_a)-1}=Rout_{s_r(t_a)}$ either
denies or accepts the request, and transmit an answer to $s_r(t_a)
= s_r(t_a-1)$. This answer contains the value $w_r(t_a+1) = 0$ if
the request is denied, and $ w_r(t_a+1)  = \lfloor
\frac{1}{2}(\rt{u}_i(t_e) - \rt{u}_{Rout_{s_r(t_a)}}) \rfloor$ if
it is accepted. There Moreover, there holds $\mathcal{P}_r(t_a+1
)=\mathcal{P}_r(t_a)$.}
%
\item{For every $t\in [t_a+1,t_f]$, there is an answer from
$Rout_{s_r(t)}(t)$ to $s_r(t)$, with the value $w_r(t) =
w_r(t_a)$. Moreover, $\mathcal{P}_r(t+1) = \mathcal{P}_r(t)
\setminus s(t)$. }
%
\item{At time $t_f$, node $r$ reads and answer from $Rout_r(t_f)
=Rout_r(t_e)$, adds $w_i(t_f)=w_i(t_a+1)$ to $\rt{u}_i$, and
returns to free mode. }
%


\end{itemize}
Besides, $\rt{u}_r(t) =\rt{u}_r(t_e)$ for every $t\in [t_e,t_f]$,
$w_r(t) = 0$ for every $t\in [t_e,t_a]$ and is constant on
$[t_a+1,t_f]$.
\end{lemma}
\begin{proof}

\emph{(b1) If $i\in \mathcal{P}_r(t)$ has an out-degree 1, then it
belongs
to $P_r(t-1)$ and $\mathcal{P}_r(t+1)$.}\\

%t+1

We prove that no node in $\mathcal{P}_r(t)\setminus\{s_r(t)\}$ can
change its $Rin$ or $Rout$ at $t-1$ or at $t$.

Let $j = Rout_i(t)\not = i$, and consider first the time $t+1$
Since $(i,j)\in G_r(t)$, there holds $Rin_j(t) = i$, and $j$ is
also in a blocked mode. There is thus no answer to request from
$j$ to $i$ at time $t$, because to send such a message, $j$ would
have had to execute "transmit answer" at time $t-1$, so that it
would be in a free mode. As a result, $i$ does not execute any
operation at time $t$ (all operations allowed in blocked mode
require a message from $Rout_i(t)=j$), and keeps its pointers
$Rin$ and $Rout$ constant from $t$ to $t+1$.

%t-1


To treat the time $t-1$, suppose now, to obtain a contradiction,
that $i$ has changed its $Rin$ or $Rout$ at time $t-1$. The node
$i$ must have been in free mode at time $t-1$, for the blocked
mode does not allow resetting $Rin$ or $Rout$ to non-empty value.
On the other hand, since $(i,j)\in G_r(t)$, there holds $Rin_j(t)
= i$, and (a1) implies that there must holds $Rout_i(t-1) =
Rout_i(t) =j$, preventing $i$ form being in a free mode at time
$t-1$.


Therefore no node in $\mathcal{P}_r(t)\setminus\{s_r(t)\}$ has
changed its $Rin$ or $Rout$ at $t-1$ or at $t$, so that
$\mathcal{P}_r(t)\setminus\{s_r(t)\}$ is present in $G_r(t-1)$ and
$G_r(t+1)$. Moreover, since by Lemma \ref{lem:descr_Gr} there
holds $Rin_r(t) =r$, and thus $Rin_r(t-1) = Rin_r(t+1)= r$, the
node $r$ has no incoming edge at time $t-1$ nor at time $t+1$. At
each of these time, there is thus a (unique) maximal path that
starts at $r$, and it contains
$\mathcal{P}_r(t)\setminus\{s_r(t)\}$.

\bigskip

\emph{(b2) Request initiation}\\

Suppose that $r$ is free at time $t-1$, and is blocked with an
in-degree 0 at time $t$. Then it must have executed "emit
request", sending a request with a value
$\rt{u}_i(t-1)=\rt{u}_i(t)$. Besides, it follows from (b1) that
its out-degree is then 0.


\bigskip


\emph{(b3) Outgoing request}\\

Suppose that there is a request from $s_r(t)$ to
$k:=Rout_{s_r(t)}(t)$. When reading the request at time $t$, $k$
can transmit it, accept it, or deny it.

Consider first the case where $k$ executes "transmit request". It
sets $Rin_k(t+1) = s_r(t)$, and it follows from (a1) that
$Rout_{s_r(t)}(t+1)= Rout_{s_r(t)}(t)= k$, so that $(s_r(t),k)$ is
an edge in the graph $G_r(t+1)$. Besides, since $s_r(t)$ was in a
blocked mode at time $t$ and remains in a block mode at time $t+1$
(for otherwise $Rout_{s_r(t)}(t+1)$ would be empty), it has
executed no operation at time $t$, and has not changed its $Rin$.
Since we have seen in (b1) that the predecessor of $s_r(t)$ (if
any) has not changed its $Rout$, this implies that
$\mathcal{P}_r(t+1)$ contains $\mathcal{P}_r(t)$ and the edge
$(s_r(t),k)$. Moreover, there is at time $t+1$ a request from $k$
to some $Rout_k(t+1)$ with exactly the same value as in the one
from $s_r(t)$ to $k$ at time $t$, which by induction means that
the value is $\rt{u}_i(t_e)$. Finally, $k$ has an out-degree 0,
for otherwise it would be the $Rin(t+1)$ of some node, which by
(a1) implies that $Rout_k(t)$ is not empty, which is impossible
since $k$ needs to be in free mode to execute "transmit request"
at time $t$. There is thus in $G_r(t+1)$ a maximal path
$\mathcal{P}_r(t) \cup k$, which starts at $r$.

Suppose now that $k$ accepts or denies the request. It sends thus
an "answer to request" message to $s_r(t)$ with either a value $0$
(request denial) or some positive value. It remains in free mode,
and does thus not enter the graph $G_r(t+1)$ nor the path
$\mathcal{P}_r(t+1)$. Besides, since $s_r(t)$ is in blocked mode,
it does not change its $Rin$ nor its $Rout$. We have also seen in
(b1) that its predecessor does not change its $Rout$ either. This
together with (b1) implies that $G_r(t+1)$ contains the edge
arriving at $s_r(t)$ in $G_r(t)$ but no edge leaving $s_r(t)$, and
thus that $\mathcal{P}_r(t)$ is a maximal path. Therefore,
$\mathcal{P}_r(t+1)=\mathcal{P}_r(t)$. Besides, $s_r(t+1) =
s_r(t)$, and there is an "answer to request" message from
$Rout_{s_r(t+1)}(t+1)$ to $s_r(t+1)$.

\bigskip


\emph{(b4) Incoming answer}\\



Suppose now that there is an "answer to a request" message from
$Rout_{s_r(t)}$ to $s_r(t)$.

If $s_r(t) =r$, then it executes "receive answer", sets
$\rt{u}_r(t+1)$ to $\rt{u}_r(t) + w_r(t)$, and reenters the free
mode. As a result, no path leave $r$ in $G_r(t+1)$.

If $s_r(t)\not =r$, and thus  $Rin_{s_r(t)} = k\not =s_r(t)$. Then
$s_r(t)$ executes "transmit answer" at time $t$: It transmits the
answer to $k$, sets its mode to "free", and leaves the path. We
know from (b1) that every node in $\mathcal{P}_r(t)\setminus
\{s_r(t)\}$ remains in a path from $r$ to $k$. Observe that $k$
cannot change its $Rout$ because it is in a blocked mode.
Therefore, no edge leaves $k$ at time $t+1$. By (b1),
$\mathcal{P}_r(t)\setminus \{s_r(t)\}$ is thus a maximal path at
time $t+1$, and starts from $r$. Besides, observe also that
$w_r(t)$ is left unchanged in the process, as the message from
$s_r(t)$ to $k$ is exactly that which arrived at $s_r(t)$.\\


\bigskip

\emph{(b5) Connection of the different parts}\\



It follows from (b1) that maximal paths of nontrivial length
leaving a given vertex $r$ do not "appear" at once, and that at
each time step, they can remain unchanged, they grow by gaining
one additional edge leaving their previously last vertex, or
shrink by losing their last edge. Since initially there is no such
path, if we observe a path $\mathcal{P}_r(t)$, there must be a
time at which it appeared. Let $t_e$ be the last such time. We
have seen in (b2) that the apparition follows the execution of
"emit request" by $r$, and that the value contained in the request
is $\rt{u}_r(t_e-1)= \rt{u}_r(t_e)$. Observe now that by (b3) or
(b4), if a some time $t$ the path does not grow, then at $t+1$
there is an "answer to request" message arriving at $s_r(t+1)$. As
a result, the path loses its last edge between $t+1$ and $t+2$,
and there is again an "answer to request" arriving at $s_r(t+2)$.
Applying this recursively, we see that the path keeps shrinking
until it disappears. Therefore, the path may have only one
increasing phase. During this phase, its length increases by 1 at
each time step, and there is a request from $s_r(t)$ to
$Rout_{s_r(t)}$. We know by Lemma \ref{lem:descr_Gr} that the path
must remain simple, so its length is bounded by $n-1$. There must
thus be a time at which the growing phase stops. Call $t_a$ the
first such time, We have seen in (b3) that if $s_r(t_a)$ is left
by a request, and if the length of $\mathcal{P}_r$ does not
increase at $t_a$, then $\mathcal{P}_r(t_a+1) =
\mathcal{P}_r(t_a)$, the node $Rout_{s_r(t_a)}(t_a)$ has denied or
accepted the request at time $t_a$, and sent an answer message
back to $s_r(t_a)$. Again, by (b4), the path then loses one edge
at each further time step, and eventually disappears at some
$t_f$. The claims on the value of the different variables follows
then from a simple recurrence argument.
\end{proof}

